CAIRN: Dynamic Fact-Intent DAGs for Multi-Agent Exploration

LLM-powered autonomous systems have demonstrated promising capabilities in mathematical reasoning, engineering, and cybersecurity. Yet how to organize these systems for effective, reliable, and sustained performance remains an open question. In this paper, we present CAIRN, a fact-intent-driven multi-agent paradigm for goal-directed exploration. CAIRN represents observations and planned investigations as a dynamic directed acyclic graph (DAG). A reasoner interprets facts to propose intents, which workers execute to produce new facts. Each intent references its supporting facts and defines a potential exploration branch. The persistent graph preserves goals, dependencies and findings across workers, supporting knowledge reuse and parallel exploration. The graph also makes execution trajectories traceable and auditable, providing a basis for human verification and intervention. We evaluate CAIRN across cybersecurity and mathematical reasoning tasks, examining task success, time to solution, and token consumption. DAG-based coordination can incur higher token costs with no observable performance gains on tasks that require little effort. However, on high-effort tasks (at least 1M tokens), we observe faster solutions in 76.5% of cases, with speedups of up to 3.08x. Moreover, as task effort increases, these time gains become more pronounced while relative token overhead declines, highlighting the potential of DAG-guided parallel exploration.

==> figures/border_light_palette.tex <==
% Shadcn-inspired paper palette: charcoal, zinc, white, and red.
\definecolor{cairnTrialAccent}{HTML}{DC2626}%
\definecolor{cairnTrialIntent}{HTML}{DC2626}
\definecolor{cairnTrialFact}{HTML}{71717A}
\definecolor{cairnTrialBoundary}{HTML}{18181B}
\ifdefined\cairnPaletteCool
  \definecolor{cairnTrialIntent}{HTML}{3D7EA6}
  \definecolor{cairnTrialFact}{HTML}{52796F}
  \definecolor{cairnTrialBoundary}{HTML}{0B2545}
\fi
\ifdefined\cairnPaletteWarm
  \definecolor{cairnTrialIntent}{HTML}{E9C46A}
  \definecolor{cairnTrialFact}{HTML}{A7C957}
  \definecolor{cairnTrialBoundary}{HTML}{A90B2F}
\fi


==> tables/benchmark_summary_rows.tex <==
% Generated by tables/update_summary_tables.py; do not edit by hand.
% Selected-run index SHA-256: ab518951c58fdc27a5a61bf6c6f699150ffda8b5f9f6fd279e7565d5beeecc13
% Resource cohort matches figures; FM runs are averaged within task first.
% Runs counts selected evaluation runs, including verified hard timeouts.
% Confirmed five-hour hard timeouts receive a 300-minute solving-time penalty.
% Effort = Direct confirmed tokens (M); ratios are means of per-task ratios.
% Time ratio = Direct/CAIRN; token ratio = CAIRN/Direct.
\multicolumn{3}{@{}l}{\textit{FrontierMath}} \\
Runs & 36 & 36 \\
Faster & 4/12 & 8/12 \\
Time (min) & 53.19 & 27.45 \\
Tokens (M) & 2.81 & 13.44 \\
\addlinespace[5pt]
\multicolumn{3}{@{}l}{\textit{Cybench}} \\
Runs\tnote{a} & 40 & 40 \\
Faster\tnote{b} & 30/40 & 10/40 \\
Time (min) & 7.31 & 8.49 \\
Tokens (M) & 0.83 & 3.22 \\


==> tables/pooled_effort_rows.tex <==
% Generated by tables/update_summary_tables.py; do not edit by hand.
% Selected-run index SHA-256: ab518951c58fdc27a5a61bf6c6f699150ffda8b5f9f6fd279e7565d5beeecc13
% Resource cohort matches figures; FM runs are averaged within task first.
% Runs counts selected evaluation runs, including verified hard timeouts.
% Confirmed five-hour hard timeouts receive a 300-minute solving-time penalty.
% Effort = Direct confirmed tokens (M); ratios are means of per-task ratios.
% Time ratio = Direct/CAIRN; token ratio = CAIRN/Direct.
\multirow{2}{*}{$\geq1$ (17)} & D & 29 & 47.20 & 3.48 & \multirow{2}{*}{1.67} & \multirow{2}{*}{3.69} \\
 & C & 29 & 25.35 & 13.56 &  &  \\
\addlinespace[0.75pt]
\multirow{2}{*}{$[0.1,1)$ (20)} & D & 30 & 5.43 & 0.35 & \multirow{2}{*}{0.66} & \multirow{2}{*}{8.66} \\
 & C & 30 & 9.13 & 2.54 &  &  \\
\addlinespace[0.75pt]
\multirow{2}{*}{$<0.1$ (15)} & D & 17 & 1.31 & 0.04 & \multirow{2}{*}{0.42} & \multirow{2}{*}{14.71} \\
 & C & 17 & 3.72 & 0.60 &  &  \\
\midrule
\multirow{2}{*}{All (52)} & D & 76 & 17.90 & 1.28 & \multirow{2}{*}{0.92} & \multirow{2}{*}{8.78} \\
 & C & 76 & 12.87 & 5.58 &  &  \\

